Magnon hydrodynamics in an atomically-thin ferromagnet

Strong interactions between particles can lead to emergent collective excitations. These phenomena have been extensively established in electronic systems, but are also expected to occur for gases of neutral particles like magnons, i.e. spin waves, in magnets. In a hydrodynamic regime where magnons are strongly interacting, they can form a slow collective density mode -- in analogy to sound waves in water -- with characteristic low-frequency signatures. While such a mode has been predicted in theory, its signatures have yet to be observed experimentally. In this work, we isolate exfoliated sheets of CrCl$_3$ where magnon interactions are strong, and develop a technique to measure its collective magnon dynamics via the quantum coherence of nearby Nitrogen-Vacancy (NV) centers in diamond. We find that the thermal magnetic fluctuations generated by monolayer CrCl$_3$ exhibit an anomalous temperature dependence, whereby fluctuations increase upon decreasing temperature. Our analysis suggests that this anomalous trend is a consequence of the damping rate of a low-energy magnon sound mode which sharpens as magnon interactions increase with increasing temperature. By measuring the magnetic fluctuations emitted by thin multilayer CrCl$_{3}$ in the presence of a variable-frequency drive field, we observe spectroscopic evidence for this two-dimensional magnon sound mode.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf -cd \"$_[0]\"" );
    }
}
